Optimized Design of A Haptic Unit for Vibrotactile Amplitude Modulation

Communicating information to users is a crucial aspect of human-machine interaction. Vibrotactile feedback encodes information into spatiotemporal vibrations, enabling users to perceive tactile sensations. It offers advantages such as lightweight, wearability, and high stability, with broad applications in sensory substitution, virtual reality, education, and healthcare. However, existing haptic unit designs lack amplitude modulation capabilities, which limits their applications. This paper proposed an optimized design of the haptic unit from the perspective of vibration amplitude modulation. A modified elastic model was developed to describe the propagation and attenuation mechanisms of vibration in the skin. Based on the model, two types of hierarchical architectural design were proposed. The design incorporated various materials arranged in multiple layers to amplify or attenuate the vibration amplitude as it traveled through the structure. An experimental platform was built to evaluate the performance of the optimized design.

==> sections/introduction.tex <==
\section{INTRODUCTION}

When robots are operated to complete tasks, in addition to understanding users’ intentions accurately, it is crucial to communicate information back to users. Providing feedback on the operation results or information obtained via sensors can achieve a closed-loop control between users and robots. For example, when individuals with physical disabilities use prosthetics to grasp objects, such as eggs, feedback about grip strength can help them maintain a stable grip while preventing the egg from being crushed. Similarly, during surgical training with robotic assistance, providing doctors with alerts after incorrect maneuvers can enhance training efficiency. Additionally, employing feedback devices in health monitoring systems can alert users to abnormal conditions, prompting timely medication intake to prevent accidents.

Feedback can be transmitted through different sensory systems. Beyond traditional visual and auditory feedback, tactile feedback encodes information into tactile sensations to stimulate the skin, which is the largest organ of the human body. Tactile perception is a basic and intrinsic human function that does not require extra effort to process information, making it generally well-received by users. It serves as a sensory substitution for individuals with visual, auditory, or physical disabilities, and plays a supportive role in education, training, gaming and social interactions\cite{to_cite}. 



related work


The rest of this paper is organized as follows. In Section \ref{sec:method}, the theoretical model is proposed, along with two optimized designs of the haptic unit. To evaluate the performance of these designs, an experimental platform is set up. Section \ref{sec:experiment} illustrates the material chosen for the design and the results of the experiments. Extended discussion is presented to validate the correctness of the theoretical model. Finally, Section \ref{sec:con} summarizes the contents of the paper.

Vibrotactile feedback stimulates human tactile sensations through vibrations to transmit information. It is achieved by motors that are adhered or bound to the skin, which encode information about the surroundings into spatiotemporal patterns. These vibrations activate the mechanoreceptors within the skin, facilitating perception, and offering advantages in terms of lightweight, wearability, and high stability. Vibrotactile feedback opens new pathways beyond visual and auditory feedback, serving as a sensory substitution for individuals with visual, auditory, or physical disabilities. Additionally, when integrated with VR/AR technologies, it plays a supportive role in education, training, gaming and social interactions.

To enhance the amount of information transmitted through the interface, researchers adopted modular design method, arranging multiple haptic units in an array to create interfaces. \cite{keef2020virtual} distributed motors on the fingertips of a vibrotactile glove, utilizing vibrations of varying amplitudes to represent the hardness of different objects within virtual environment. Similarly, \cite{garcia2017evaluation} positioned motors at various locations across the torso to develop a vibration jacket, which simulates explosion scenarios in VR games through vibration. These designs integrate haptic units into garments with a hard-wired structure, resulting in a bulky size, heavy weight, and reduced wearability, thereby limiting their applications\cite{zhu2020development}.

A more compact and wearable interface can be achieved by arranging haptic units adjacently and connecting them via a flexible circuit board. Each haptic unit consists of a vibratory motor, circuits, and a power supply module, and is controlled by a microcontroller for spatiotemporal encoding. \cite{jung2022wireless} arranged 36 eccentric rotating mass (ERM) motors in an array with a spacing of 13 mm. A double-sided flexible printed circuit board (FPCB) supports the actuators and associated control circuits, with a two-layer soft and stretchable silicone elastomer featuring a hollow structure forming the encapsulation structure. \cite{jung2021skin} utilized a similar structure in their design, where the haptic actuator has a diameter of 8 mm, the haptic unit has a diameter of 18 mm, and the distance between adjacent haptic units is 21 mm. 

Although miniaturized integrated designs can produce richer sensations, they are susceptible to the threat of mechanical crosstalk. Typically, vibration interfaces use soft materials like silicone for encapsulation, which possess a certain degree of elasticity. Additionally, human skin acts as a multi-layered viscoelastic medium, which allows vibrations from a single unit to spread to a significantly larger surrounding area, causing mechanical crosstalk that can interfere with the user’s ability to discern the number and location of vibrating motors, thus limiting the effective transmission of information\cite{kim2024wirelessly}. 

To optimize the design of vibrotactile interfaces, researchers have conducted a series of studies on the mechanical properties of skin, the vibration characteristics of motors adhered to the skin, and the propagation mechanism of waves within the skin through theoretical modeling, finite element analysis and physical experiments. 


==> sections/related_work.tex <==
\section{RELATED WORK}

The skin is a multi-layered viscoelastic medium that consists of the epidermis, dermis, and hypodermis\cite{liu2017lab}. Its parameters include the elasticity modulus, density, Poisson's ratio, and viscosity\cite{yazdi2022mechanical}. Researchers conducted experiments and simulations to investigate the mechanisms of each skin layer when stimulated by vibrations at different frequencies\cite{moore1970survey}. Gierke H E V et al. measured the acoustic impedance of the skin on the thighs and forearms and found that at and below a motor vibration frequency of approximately 150Hz, the skin primarily exhibits elasticity, with viscosity having a minor effect on wave propagation\cite{von1952physics}. As the vibration frequency increases, the skin exhibits more viscous behavior. This finding is consistent with results from studies on other parts of the human body\cite{wiertlewski2012mechanical}. Consequently, researchers mostly use elastic models to study the propagation of waves induced by vibration motors in the skin\cite{yu2019skin,kim2023mechanics,kim2024wirelessly}. 

On the basis of linear elastic model, in order to describe the propagation and attenuation mechanisms more precisely, researchers also considered viscosity when modeling the skin. Andrews J et al. developed a four-layer modified elastic model consisting of the stratum corneum, soft tissue, cortical bone, and cancellous bone to analyze the propagation patterns of surface waves during contact interaction\cite{andrews2020universal}. Modified elastic model incorporates an exponential term into the linear elastic model to characterize the skin's viscosity and study the propagation and attenuation of vibration waves in the skin. Compared to the linear elastic model, the modifies elastic model considers material attenuation on the basis of geometric attenuation, resulting in a better fit. Amaied E et al. created a cross-sectional finite element model of the fingertip to study the impact of age on tactile perception. A linear elastic model is used to represent the fingernail and bone, while a multi-layer viscoelastic model is used for the skin\cite{amaied2015aging}.

Based on the understanding of skin characteristics, researchers optimized the design of vibrotactile interfaces. Yu X et al. innovatively designed a vibration motor featuring a cantilever beam structure that can induce uneven vibrations of different amplitudes in various directions along the skin surface\cite{yu2019skin}. By optimizing the orientation of the haptic units, mechanical crosstalk between adjacent units was minimized. However, this method is only applicable to the innovative haptic units proposed in the paper. Kim J H et al. found that skin sensitivity varies with temperature; therefore, they incorporated a temperature module into the vibration interface to reduce the two-point threshold by increasing skin temperature. Additionally, the inclusion of the temperature module resulted in an increase in motor height. A three-dimensional digital image correlation method was used to generate spatiotemporal maps of the underlying skin model deformations, showing that as the height of the acrylic material beneath the vibration motor increased, the displacement around the motor on the skin significantly decreased. This further addressed the issue of mechanical crosstalk in array-based vibration interfaces. However, whether increasing the height of the vibration motor or incorporating a temperature module into the interface, both approaches resulted in an increase in the size of the array-based vibration interface.

Existing tactile unit designs lack amplitude modulation capabilities. When these units are applied to body areas with a lower density of mechanoreceptors, a greater number of units are required, leading to increased interface volumes. Additionally, because both the encapsulation and skin are elastic, vibrations from a single unit tend to spread over a larger area, making the interface susceptible to mechanical crosstalk. 

This paper establishes a multi-layer medium modified elastic model based on an eccentric rotating mass motor, characterizing the propagation and attenuation mechanisms of vibrations induced by haptic units on the skin surface. From the perspective of amplitude modulation, optimization schemes are proposed to amplify or reduce the amplitude of vibration waves induced by the haptic unit adhered to the skin. The optimized design is adhered to a skin phantom and the amplitude was measured by a laser doppler vibrometer. The rest of this paper is organized as follows. In Section III, the theoretical model is proposed, along with two optimized designs of the haptic unit. To evaluate the performance of these designs, an experimental platform is set up. Section IV illustrates the material chosen for the design and the results of the experiments. Section V presents the extended discussion and validates the correctness of the theoretical model. Finally, Section VI summarizes the contents of the paper.
